The COBE Normalization of CMB Anisotropies

With the advent of the COBE detection of fluctuations in the Cosmic Microwave Background radiation, the study of inhomogeneous cosmology has entered a new phase. It is now possible to accurately normalize fluctuations on the largest observable scales, in the linear regime. In this paper we present a model-independent method of normalizing theories to the full COBE data. This technique allows an extremely wide range of theories to be accurately normalized to COBE in a very simple and fast way. We give the best fitting normalization and relative peak likelihoods for a range of spectral shapes, and discuss the normalization for several popular theories. Additionally we present both Bayesian and frequentist measures of the goodness of fit of a representative range of theories to the COBE data.

==> cobenorm_erratum.tex <==
\magnification1200

%This defines \simgreat and \simless.
\newbox\grsign \setbox\grsign=\hbox{$>$} \newdimen\grdimen \grdimen=\ht\grsign
\newbox\simlessbox \newbox\simgreatbox
\setbox\simgreatbox=\hbox{\raise.5ex\hbox{$>$}\llap
     {\lower.5ex\hbox{$\sim$}}}\ht1=\grdimen\dp1=0pt
\setbox\simlessbox=\hbox{\raise.5ex\hbox{$<$}\llap
     {\lower.5ex\hbox{$\sim$}}}\ht2=\grdimen\dp2=0pt
\def\simgreat{\mathrel{\copy\simgreatbox}}
\def\simless{\mathrel{\copy\simlessbox}}
\def\simlt{\simless}

\centerline{{\bf Erratum}}

\vskip 0.1in

\centerline{The COBE Normalization of CMB Anisotropies}

\centerline{Martin White \& Emory Bunn}

\centerline{Ap.~J.~{\bf 450}, 477 (1995)}

\vskip 0.2in

In tables 1 \& 2 the quoted values of $\Delta^2$ and $\sigma_8$ assume a
tensor-to-scalar ratio $C_2^{T}/C_2^{S}=7(1-n)$.  This is the correct lowest
order (in an expansion in $1-n$) expression for the tensor-to-scalar ratio
for $\Omega_0=1$.  However the projection from the $k$-space inflationary
prediction onto the quadrupole, i.e.~$\ell=2$ mode, has a dependence on
$\Omega_\Lambda$ and $n$, which was neglected in calculating the entries in
the tables.  The ``correction factor'', $f_{T/S}(\Omega_\Lambda,n)$, defined
through
$$
C_2^T/C_2^S = 7\,(1-n)\ f_{T/S}(\Omega_\Lambda,n)
$$
can be well fit by
$$
f_{T/S}(\Omega_\Lambda,n) = 0.97-0.58(1-n) + 0.25\Omega_\Lambda
    - \left[ 1-1.1(1-n)+0.28(1-n)^2\right]\Omega_\Lambda^2 \quad .
$$
This expression includes both the full $n$ dependence (i.e.~beyond leading
order in $1-n$) of power-law inflation, for which exact expressions are
available, and the ISW contribution to $C_2^S$.  To good approximation the
values of $\Delta^2$ quoted in the tables should be multiplied by
$$
{1+7(1-n)\over 1+7(1-n)f_{T/S}}
$$
and the values of $\sigma_8$ by the square root of this.  For reasonable values
of $\Omega_\Lambda$ and $n$ this amounts to a $\simlt10\%$ correction.

\end

